Optical spin glasses: a new model for glassy systems

The aim of this work is to prove that it is possible to realise an optical system which produces as output a light intensity that can be expressed in the same mathematical form of the spin glass Hamiltonian. The optical system under study is controlled through an adaptive optics device composed by millions of switchable mirrors in an ON and OFF position. These user controlled mirrors are playing the role of the spin states. Furthermore, such optical system can be used to run simulations and, applying the same Metropolis Monte Carlo algorithm used in computer simulations, extract the quantities of interest for Spin Glass physics. The proposed system has a great advantage over existing computer-based spin glass simulations: the simulation step has no scaling dependence on the total number of spins $N$ and the whole simulation has a linear dependence on $N$, due to the fact that we want to keep the number of moves per spin constant. This should be compared to the $N^2$ dependence of a single Monte Carlo move in computer simulation, which yields a global N3 dependence. Some experimental problems limit such advantage, but are partially addressed at the end of the presentation.

==> spinglass.tex <==
\chapter{Mapping two problems on one another}

\epigraph{If we expand our experience into wilder and wilder regions of experience - every once in a while - we have these integrations when everything's pulled together into a unification, in which it turns out to be simpler than it looked before.}{\textit{Richard Feynmann}}
\section{The hamiltonian of the optical spin glass}
Let's now suppose that the incident wave on the DMD is a monochromatic plane wave travelling along the $z$ direction; we can write it as:
\begin{equation}
\vec{E}_{in} = \vec{\epsilon}\,E_0\,e^{i\left(kz-\omega t\right)}
\end{equation}

In which the laser wave is assumed perfectly coherent, in time and space. After being reflected by the dmd, we have a variable $\sigma$ in which we encode the activation state of the dmd pixel. The reflected wave will be:
\begin{equation}
\vec{E}_{out}=\vec{\epsilon}\,E_0\,e^{i\omega t}\,e^{ikz}\,\sigma\left(x,y\right)
\end{equation}
and, because the dmd is made up by pixels, the function $\sigma$ can be discretise and expressed as a function of an index $i$:
\begin{equation}
\vec{E}_0\left(\vec{r}_i\right)=\vec{\epsilon}\,E_0\,e^{i\omega t}\,e^{ikz_i}\,\sigma\left(x_i,y_i\right)=\vec{\epsilon}\,E_0\,e^{i\omega t}\,e^{ikz_i}\,\sigma_i
\end{equation}
in which $\sigma_i=\{0,1\}$ depending on the activation state of the i-th pixel.\newline

We now want to enforce the \emph{autoconsistency} equations for the electric field in a scattering medium, namely the relation:
\begin{equation}\label{autoconsistency_naive}
\vec{E}_1=\vec{E}_0+\sum_i\{\mbox{scattered spherical waves } S_i\}
\end{equation}
which expresses the resulting electric field in terms of all the fields generated in the scattering process in the sample.
More formally, the condition (\ref{autoconsistency_naive}) can be written in terms of the \emph{dipole propagator} in the following way:
\begin{equation}
\vec{E}_1=\vec{E}_0+\sum_i\,\mymatrix{T}_{1i}\,\alpha_i\,\vec{E}_i
\end{equation}
The dipole propagator can be written \cite{DipolePropagator} as:
\begin{equation}
\mymatrix{T}_{ij}\left(\vec{r}\omega\right)=\frac{1}{4\pi\epsilon_0}\left[\left(\frac{\omega n}{c}\right)^2+\frac{\partial^2}{\partial r_i\,\partial r_j}\right]\,\frac{e^\frac{i\omega nr}{c}}{r}
\end{equation}
Hence, in general, we can write, for every pixel of the dmd:
\begin{equation}
\vec{E}\left(\vec{r}_i,t\right)=\vec{E}_0\left(\vec{r}_i,t\right)+\sum_j\mymatrix{T}_{ij}\;\alpha_j\,\vec{E}_0\left(\vec{r}_j,t\right)
\end{equation}
Il tempo è uguale per tutti, cioè non c'è ritardo di fase oltre a quello impresso dal SLM, perché i fascio laser è spazialmente e temporalmente coerente). Quindi facciamo cadere la dipendenza temporale:
\begin{equation}
\vec{E}\left(\vec{r}_i\right)=\vec{E}_0\left(\vec{r}_i\right)+\sum_j\mymatrix{T}_{ij}\;\alpha_j\,\vec{E}_0\left(\vec{r}_j\right)
\end{equation}
O, alleggerendo la notazione:
\begin{equation}\label{recurrence}
\vec{E}_i=\vec{E}_{0i}+\sum_j\mymatrix{T}_{ij}\;\alpha_j\,\vec{E}_j
\end{equation}
Ora espandiamo l'espressione del campo per ricorrenza, ovvero scrivendo $\vec{E}_j$ in funzione di $\vec{E}_{oj}$ come nell'Equazione (\ref{recurrence}):
\begin{align}
\notag\vec{E}_i &= \vec{E}_{0i} +\sum_j\mymatrix{T}_{ij}\;\alpha_j\,\left[\vec{E}_{0j}+\sum_k\mymatrix{T}_{jk}\;\alpha_k\,\vec{E}_k\right]=\\
\notag&=\vec{E}_{0i}+\sum_j\mymatrix{T}_{ij}\;\alpha_j\,\vec{E}_{0j} +\sum_{j,k}\mymatrix{T}_{ij}\;\mymatrix{T}_{jk}\;\alpha_j\,\alpha_k\,\vec{E}_k=\\
\notag&=\sum_j\delta_{ij}\,\vec{E}_{0j}+\sum_j\mymatrix{T}_{ij}\;\alpha_j\,\vec{E}_{0j} +\sum_{j,k}\mymatrix{T}_{ij}\;\mymatrix{T}_{jk}\;\alpha_j\,\alpha_k\,\vec{E}_k=\\
\notag&=\sum_j\delta_{ij}\,\vec{E}_{0j}+\sum_j\mymatrix{T}_{ij}\;\alpha_j\,\vec{E}_{0j} +\sum_{k,j}\mymatrix{T}_{ik}\;\mymatrix{T}_{kj}\;\alpha_k\,\alpha_j\,\vec{E}_j=\\
\notag&=\sum_j\delta_{ij}\,\vec{E}_{0j}+\sum_j\mymatrix{T}_{ij}\;\alpha_j\,\vec{E}_{0j} +\sum_{k,j}\mymatrix{T}_{ik}\;\mymatrix{T}_{kj}\;\alpha_j\,\alpha_k\,\vec{E}_{0j}+...=\\
\vec{E}_i&=\sum_j \mymatrix{M}_{ij}\;\vec{E}_{0j}
\end{align}
in cui la nuova matrice $\mymatrix{M}$ è definita come:
\begin{equation}
\mymatrix{M}_{ij}=\delta_{ij}+\mymatrix{T}_{ij}\;\alpha_j+\sum_k\mymatrix{T}_{ik}\;\mymatrix{T}_{kj}\;\alpha_j\,\alpha_k+...
\end{equation}
Otteniamo quindi una scrittura di $\vec{E}_i$ buona per continuare il calcolo:
\begin{equation}
\vec{E}_i=\sum_j\mymatrix{M}_{ij}\;\vec{E}_{0j} = \sum_j\mymatrix{M}_{ij}\;\hat{\epsilon}\,E_0e^{i\omega t}e^{ikz}\sigma_j
\end{equation}
Il segnale che giunge sul campione è una porzione del campo proveniente da punto $i$-esimo, ed è quindi $\sim\alpha_i\,\vec{E}_0$. Questa sarà la mia funzione \emph{energia}:
\begin{align}
\notag S_i&=\frac{\Delta\Omega}{4\pi}\,\alpha^2_i\,\left|\vec{E}_i\right|^2=\\
S_i&=\frac{\Delta\Omega}{4\pi}\alpha^2E_0^2\sum_{j,j'}\left(\mymatrix{M}_{ij}\,\hat\epsilon\right)\cdot\left(\mymatrix{M}_{ij'}\,\hat\epsilon\right)\,e^{ik(z_j-z_{j'})}\sigma_j\,\sigma_{j'}
\end{align}
Ora lasciamo cadere l'indice $i$, che serve solamente a dirci che tutto quello che è stato detto dipende dal punto che si prende come target. Otteniamo:
\begin{align}
\notag S&=\frac{\Delta\Omega}{4\pi}\alpha^2E_0^2\sum_{j,j'}J_{jj'}\sigma_j\sigma_{j'}=\\
S&=S_0 \sum_{i,j}J_{ij}\,\sigma_i\,\sigma_j\label{hamiltonian}
\end{align}
in cui abbiamo trovato le relazione fra e due grandezze dell'hamiltoniana di spin glass e le quantità fisiche in gioco:
\begin{align}
S_0&=\frac{\Delta\Omega}{4\pi}\alpha^2E_0^2\\
J_{ij}&=e^{ik(z_i-z_j)}\left(\mymatrix{M}_{0j}\,\hat\epsilon\right)\cdot\left(\mymatrix{M}_{0j'}\,\hat\epsilon\right)=\\
\notag&=e^{ik(z_i-z_j)}\sum_{\alpha,\beta,\gamma}\epsilon_\alpha\,\epsilon_\beta\,M_{oi}^{\alpha\beta}\,M_{0j}^{\gamma\beta}
\end{align}

\noindent Vogliamo ora mostrare che la matrice $\mymatrix{J}$ è simmetrica. Dobbiamo mostrare quindi che $J_{ij}~=~J_{ji}$ $\forall (i,j)$. Per dimostrarlo facciamo riferimento alla Figura (\ref{dephase}) e consideriamo i due raggi incidenti sui pixel $i$-esimo e $j$-esimo. Essi si trovano in fase prima della riflessione sul SLM per le proprietà di coerenza della sorgente laser. Dopo la riflessione essi assumono uno sfasamento di $0$ o $\pi$ radianti a seconda dello stato del pixel corrispondente. Lo scatteratore aggiunge un altro ritardo di fase $e^{i\theta_k}$ che è funzione del solo pixel che produce il raggio 

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=10cm]{scatterator.eps}
\caption{Sfasamenti subiti da due raggi provenienti dal laser.}
\label{dephase}
\end{center}
\end{figure}
\clearpage

